PrimeQA: The Prime Repository for State-of-the-Art Multilingual Question Answering Research and Development

The field of Question Answering (QA) has made remarkable progress in recent years, thanks to the advent of large pre-trained language models, newer realistic benchmark datasets with leaderboards, and novel algorithms for key components such as retrievers and readers. In this paper, we introduce PRIMEQA: a one-stop and open-source QA repository with an aim to democratize QA re-search and facilitate easy replication of state-of-the-art (SOTA) QA methods. PRIMEQA supports core QA functionalities like retrieval and reading comprehension as well as auxiliary capabilities such as question generation.It has been designed as an end-to-end toolkit for various use cases: building front-end applications, replicating SOTA methods on pub-lic benchmarks, and expanding pre-existing methods. PRIMEQA is available at : https://github.com/primeqa.

==> repository4.tex <==
\section {PrimeQA Repository}

\begin{figure*}
 %\includegraphics[width=\textwidth,height=10cm]{images/reasoning_arch.pdf}
 \includegraphics[width=2\columnwidth]{images/repo.pdf}
 \caption{PrimeQA Repository: The core components available in PrimeQA}
 \label{fig:pqa_tree}     
\end{figure*}

\begin{table*}[t]\small
\centering
\begin{tabular}{lll}
\toprule
\textbf{Models}	&	\textbf{Applications}	&	\textbf{Datasets}		\\
\midrule
              \multicolumn{3}{c}
              {\textbf{Retriever}}		\\
\midrule
BM25 \cite{RobertsonBM25}	&	Dr.DECR	\href{https://nlp.cs.washington.edu/xorqa/}{*} \cite{li-etal-2022-learning-cross} &	NQ			\\
DPR	\cite{karpukhin-etal-2020-dense} &		&	XOR-TyDi \cite{asai-etal-2021-xor}			\\
ColBERT	\cite{santhanam-etal-2022-colbertv2} &		&		ELI5		\\
\midrule
             \multicolumn{3}{c}{\textbf{Reader}}	
             \\
 \midrule
General MRC	&	ReasonBert	&	SQuAD \cite{rajpurkar-etal-2016-squad}		\\
FiD	&	MIT-QA	&	TyDiQA \cite{tydiqa}		\\
Boolean\href{https://ai.google.com/research/tydiqa}{*} \cite{https://doi.org/10.48550/arxiv.2206.08441} 
  &	OmniTab	&	NQ \cite{nq47761}	\\
	Lists	&	MuMuQA	&	ELI5			\\
Tapas	&		&	WikiSQL			\\
Tapex	&		&	SQA			\\
	&		&	WTQ			\\
	&		&	DocVQA			\\
    & & HybridQA \\
\midrule
\multicolumn{3}{c}{\textbf{Question Generation}}		\\
\midrule
Table QG	&	QVE	&	WikiSQL			\\
Passage QG	&		&	SQuAD			\\
Hybrid QG	&		&	TyDiQA			\\
Entity Grounded QG	&		&				\\
 \bottomrule
\end{tabular}
\caption{ A non-exhaustive list of the models available on our HuggingFace model hub \url{https://huggingface.co/PrimeQA}, applications, and tasks supported by our core components. * SOTA Leaderboard systems.
}
\label{tab:models_apps_tasks}
\end{table*}

The PrimeQA repository, a ``one stop shop" for SOTA QA research, combines a development process governed by the following design principles: 

%The PrimeQA repository is the one stop solution for state of the art QA research across different user groups. It is designed to build complex and robust end-to-end models and enable the community to use, extend and combine core QA components as plug and play building blocks. The development process is governed by the following design principles: 

\noindent$\bullet$ \textbf{Reproducible:} Researchers can reproduce and extend results reported in publications
%Our framework enables the researcher to extend existing approaches 
and combine them with other available SOTA algorithms.
%not in a silo custom environment but in a reusable framework that lets the researcher extend the research work further by combining with other available state-of-art techniques.

\noindent$\bullet$ \textbf{Customizable:} PrimeQA allows users to customize SOTA models for their own applications, which often entails fine-tuning on custom data which, in tuen, can be used with a custom processor or by converting the data into a supported data format. 

\noindent$\bullet$ \textbf{Reusable:} Our focus is to make it very easy for a developer to use any of the existing models in PrimeQA in their application or software with just minimal additional code lines.

$\bullet$ \textbf{Accessible:} We are tightly integrated with Huggingface datasets and their model hub allowing users to easily plug in compatible datasets and models.


\subsection{PrimeQA: Entry Points}

To support the needs of different users in the QA community, we provide different entry points to access the repository as shown in Figure~\ref{fig:pqa_tree}.

\bullet{run-component.py:} Reseachers can make the most of PrimeQA by using the Top Level Scripts, run-\textit{component}.py, to reproduce the results as we all train, finetune, evaluate these models on own custom data. \eat{and also customize each component. Using these scripts, users can reproduce SOTA results. Researchers and advanced NPL developers can use these scripts to integrate their custom datasets and models during development. }

\bullet{Notebooks:} The Notebooks demonstrate how to use built-in classes in PrimeQA to perform the various tasks of PrimeQA components and is useful for developers, researchers and contributors who want to reuse and extend PrimeQA functionalities.

\bullet{Inference APIs:}The Inference API is mainly meant for developers and shows how to use a PrimeQA component on own data with minimal lines of code. The inference APIs can be initialized with the pre-trained PrimeQA models provided in the HuggingFace hub or with a custom model that has been trained for a specific use case.  

\bullet{Service Layer:} The service layer helps developers to set up an end-to-end QA system quickly by providing a wrapper around the core components that expose an endpoint and an API. 

\bullet{UI:} UI is meant of end-users, including non technical layman who wants to use PrimeQA services interactively. 

\subsection{Components and Pipeline}

Figure~\ref{fig:pqa_tree} shows a diagram of the  PrimeQA repository. 
The repository is centered around three core components: the Retriever, the Reader and the Question Generator. The components can be used stand-alone or can be combined into a pipeline object to obtain an end-to-end QA system. All components are implemented on top of existing AI libraries such as the HuggingFace Transformers and Datasets, Pyserini and FAISS. 
\eat{
To support the needs of different users in the QA community, we provide different entry points to access the repository.

The Top Level Scripts, run-\textit{component}.py, can be used to train and evaluate each component. Using these scripts, users can reproduce SOTA results. Researchers and advanced NPL developers can use these scripts to integrate their custom datasets and models during development. 
The Notebooks provide code snippets showing details of our core components and pointers on how our components can be extended to support new functionality.

The Inference API makes it easy for all developers to use a QA system. The inference APIs can be initialized with the pre-trained PrimeQA models provided in the HuggingFace hub or with a custom model that has been trained for a specific use case.  

The services provide a wrapper around the core components that expose an endpoint and an API. The services make it easy to show case the end-to-end QA system, including the custom components, in a demo.
}
\subsubsection{Retriever}

In a open retrieval QA framework, the retriever component receives the question and retrieves the relevant documents, or the context, from a large corpus.
PrimeQA supports both sparse and dense representation retrieval engines. 

The sparse IR engine is based on Pyserini, and uses the BM25 ranking formula \cite{RobertsonBM25}. 

There are two dense IR engines supported: ColBERT \cite{santhanam-etal-2022-colbertv2}, and Direct Passage Retrieval (DPR), \cite{karpukhin-etal-2020-dense}. Both ColBERT and DPR use trained question and passage encoders. These encoders are usually initialized with pre-trained language models including BERT and XLM-RoBERTA.  
PrimeQA users can train and create indexes with ColBERT and DPR systems using their custom training data and corpora. Pre-trained models for ColBERT, including the SOTA DR.DECR model \cite{li-etal-2022-learning-cross} are available in the HuggingFace model hub.



\subsubsection{Reader}

The reader is a multilingual Machine Reading Comprehension (MRC) component that will provide an answer given a question and a context. Traditionally the context can be a paragraph or document.  Our reader can be used to train, evaluate, and predict for MRC. It works with extractive and generative models extended from HuggingFace transformers for QA. 

\noindent\textbf{Extractive:} The extractive reader is a pointer network described in \cite{}. It can be initialized with different pre-trained language models including BERT, multilingual BERT, RoBERTa and XLM-RoBERTa. The extractive reader supports general MRC but also special features such as boolean and list questions. Examples of extractive reader models and tasks can be seen in Table~\ref{tab:models_apps_tasks}. We provide readers trained on popular QA datasets, such as SQuAD, Natural Questions and TyDiQA, in the HuggingFace model hub

PrimeQA also supports and extractive multi-model reader for question answering over hybrid context of table and text.\avi{Briefly a sentence about Tapex, Tabert, Omnitab, MITQA for hybrid and ottqa. - jaydeep and vk add this one. Riyaz can add about Docvqa - but only a sentence with a citation.}
%\subsubsection{Question Answering over Hybrid Context of Table and Text}
%\vk{WIP}\\
%PrimeQA supports training models for question answering over hybrid context of table and text. 

\noindent\textbf{Generative:} The generative reader is a Fusion in Decoder model. The FiD model is initialized with pre-trained seq2seq models including BART and T5. With FiD, the question and the retrieved passages are used to generate a complex multi-sentence answer. The FiD reader is used for long form question answering on the ELI5 task. 

\subsubsection{Question Generation}
PrimeQA supports question generation (QG) with an aim to help in domain adaptation for existing reader models, as ~\cite{t3qa} had empirically demonstrated. PrimeQA extends the same seq-to-seq generation architecture from ~\cite{t3qa} for question generation across different modalities i.e. text, table, as well as hybrid context over table and text.
\noindent\textbf{Passages:} PrimeQA has a multilingual passage QG model uploaded in HuggingFace modelhub which is trained on tydiqa ~\cite{tydiqa} dataset using T5~\ref{t5} based seq-to-seq generator. One can easily train the qg model on other datasets such as squad ~\cite{} by simply changing a parameter in a well documented easy to use python script \href{https://github.com/primeqa/primeqa/tree/main/primeqa/qg}{\texttt{run\_qg.py}}. This python script also supports finetuning the qg model on user's custom data or use PrimeQA's \href{https://github.com/primeqa/primeqa/tree/main/notebooks/qg}{easy inference APIs} to generate question-answer pairs in users custom domain.

\noindent\textbf{{Tables:}
\noindent\textbf{{Hybrid Context}

\subsection{Pipelines: building on PrimeQA Core}

The pipeline component is used to create an end-to-end QA system and combines the retrieval and reader.
Any type of retrieval and reader component can be integrated in a pipeline object in a plug and play fashion.
The QA pipeline receives a question and uses the retrieval component to obtain supporting passages/context.
Once the supporting passages are available, the reader component will produce an answer.
If the pipeline uses an extractive reader, the answer is extracted from one of the supporting passages.
If the pipeline used a generative reader, such as FiD, the retrieved passages are used to generate a complex multi-sentence answer.

\noindent\textbf{Pipeline for QA over Hybrid Context of Table and Text:}
PrimeQA supports question answering over hybrid context of table and text via \textit{table splitter}, \textit{row retriever}, \textit{passage filter} and \textit{reader with re-ranker}. The \textit{row retriever} is a BERT based model trained using multi-instance loss. The \textit{reader+re-ranker} is based on PrimeQA mrc and trained using multi-answer loss function.

\eat{
 - start with ORQA as the main usecase, primeqa should provide plug n play components. 
 - to make it seamless, we follow below design principles for
  reproducibility 
  customizability
  reusability 
 }
